Understanding and predicting cadence effects in the characterization of exoplanet transits

We investigate the effect of observing cadence on the precision of radius ratio values obtained from transit light curves by performing uniform Markov Chain Monte Carlo fits of 46 exoplanets observed by the Transiting Exoplanet Survey Satellite (TESS) in multiple cadences. We find median improvements of almost 50% when comparing fits to 20s and 120s cadence light curves to 1800s cadence light curves, and of 37% when comparing 600s cadence to 1800s cadence. Such improvements in radius precision are important, for example, to precisely constrain the properties of the radius valley or to characterize exoplanet atmospheres. We also implement a numerical Information Analysis to predict the precision of parameter estimates for different observing cadences. We tested this analysis on our sample and found it reliably predicts the effect of shortening observing cadence with errors in the predicted % precision of <0,5% for most cases. We apply this method to 157 TESS object of interest that have only been observed with 1800s cadence to predict the precision improvement that could be obtained by reobservations with shorter cadences and provide the full table of expected improvements. We report the 10 planet candidates that would benefit the most from reobservations at short cadence. Our implementation of the Information Analysis for the prediction of the precision of exoplanet parameters, Prediction of Exoplanet Precisions using Information in Transit Analysis (PEPITA) is made publicly available.

==> long_improvements_table.tex <==
\begin{table}
\centering
\caption{Predictions for all the planet candidates considered in order of decreasing improvements to the radius ratio precision.}
\begin{tabular}{rrrr}
\toprule
    TOI &  20s Improv. [\%] &  120s Improv [\%] &  600s Improv [\%] \\
\midrule
1677.01 &            77.93 &            77.71 &            72.96 \\
2784.01 &            70.94 &            70.35 &            54.13 \\
3786.01 &            66.84 &            66.79 &            65.89 \\
1701.01 &            66.33 &            65.00 &            40.53 \\
2578.01 &            65.54 &            65.11 &            57.89 \\
4197.01 &            52.43 &            51.77 &            42.86 \\
5577.01 &            51.98 &            51.19 &            36.91 \\
5654.01 &            51.12 &            50.77 &            43.22 \\
3719.01 &            50.81 &            50.40 &            42.10 \\
2341.01 &            50.31 &            49.65 &            35.63 \\
3788.01 &            48.18 &            47.77 &            41.61 \\
3859.01 &            45.68 &            45.36 &            39.05 \\
1658.01 &            45.34 &            45.12 &            40.67 \\
3765.01 &            44.92 &            44.41 &            37.35 \\
3972.01 &            44.66 &            43.91 &            35.28 \\
3762.01 &            43.91 &            43.82 &            42.12 \\
3805.01 &            43.89 &            43.45 &            34.29 \\
3571.01 &            42.28 &            41.77 &            36.00 \\
5122.01 &            41.35 &            41.24 &            37.08 \\
3651.01 &            41.06 &            40.87 &            36.97 \\
3670.01 &            40.86 &            40.37 &            27.25 \\
5702.01 &            40.63 &            39.43 &            21.96 \\
5579.01 &            40.40 &            40.01 &            35.41 \\
3792.01 &            39.86 &            38.43 &            18.70 \\
3642.01 &            38.47 &            38.07 &            32.29 \\
3747.01 &            38.12 &            37.80 &            32.22 \\
2533.01 &            38.05 &            37.37 &            27.98 \\
3686.01 &            37.85 &            37.23 &            30.25 \\
3118.01 &            36.73 &            36.21 &            27.59 \\
3654.01 &            36.64 &            35.99 &            25.64 \\
1521.01 &            35.61 &            35.31 &            31.37 \\
3737.01 &            35.01 &            34.56 &            28.25 \\
5644.01 &            34.99 &            34.85 &            32.27 \\
5762.01 &            34.55 &            34.36 &            30.76 \\
1559.01 &            33.78 &            33.52 &            29.56 \\
1655.01 &            33.11 &            32.64 &            19.57 \\
3946.01 &            32.68 &            32.31 &            26.80 \\
3699.01 &            32.56 &            32.12 &            26.06 \\
2395.01 &            32.51 &            32.16 &            26.66 \\
3976.01 &            32.27 &            31.87 &            25.36 \\
 302.01 &            31.99 &            31.82 &            28.62 \\
5686.01 &            30.82 &            30.28 &            23.28 \\
3999.01 &            30.51 &            30.21 &            25.92 \\
3842.01 &            30.37 &            29.77 &            22.39 \\
2790.01 &            30.10 &            29.60 &            23.17 \\
3727.01 &            29.55 &            29.28 &            25.29 \\
3755.01 &            28.99 &            28.42 &            20.36 \\
4199.01 &            28.83 &            28.35 &            21.44 \\
3795.01 &            28.36 &            27.20 &            13.41 \\
5754.01 &            28.33 &            28.21 &            25.84 \\
3920.01 &            28.22 &            28.08 &            25.49 \\
3829.01 &            27.98 &            27.62 &            23.62 \\
2033.01 &            27.68 &            27.48 &            23.89 \\
4231.01 &            27.33 &            27.01 &            21.76 \\
3763.01 &            26.47 &            25.90 &            18.67 \\
5656.01 &            26.26 &            25.21 &            12.57 \\
3573.01 &            26.16 &            26.02 &            23.13 \\
5669.01 &            26.03 &            25.60 &            19.59 \\
3703.01 &            25.85 &            25.62 &            21.88 \\
3660.01 &            24.22 &            24.06 &            21.01 \\
5458.01 &            23.95 &            23.76 &            21.17 \\
3773.01 &            23.89 &            23.73 &            20.69 \\
3671.01 &            23.69 &            23.53 &            20.19 \\
5482.01 &            23.44 &            23.28 &            20.05 \\
5479.01 &            23.18 &            23.03 &            21.51 \\
3335.01 &            22.66 &            22.15 &            14.94 \\
3800.01 &            22.55 &            22.26 &            18.25 \\
3664.01 &            22.35 &            22.06 &            17.47 \\
1536.01 &            22.21 &            22.14 &            20.91 \\
4204.01 &            22.18 &            21.72 &            17.34 \\
3980.01 &            22.17 &            22.07 &            20.09 \\
5773.01 &            21.68 &            21.25 &            15.42 \\
3768.01 &            21.61 &            21.27 &            16.62 \\
3640.01 &            21.34 &            21.20 &            18.72 \\
3645.01 &            21.16 &            20.68 &            14.60 \\
3769.01 &            21.09 &            20.88 &            17.27 \\
2350.01 &            21.04 &            20.24 &             6.64 \\
5749.01 &            20.72 &            20.45 &            16.05 \\
5459.01 &            20.65 &            20.52 &            17.96 \\
2036.01 &            20.57 &            20.39 &            17.81 \\
3744.01 &            20.13 &            19.99 &            17.60 \\
5681.01 &            19.99 &            19.64 &            11.13 \\
1605.01 &            19.92 &            19.78 &            17.28 \\
3733.01 &            19.72 &            19.60 &            17.39 \\
2060.01 &            19.65 &            19.57 &            18.05 \\
3721.01 &            19.29 &            19.04 &            16.00 \\
5618.01 &            18.86 &            18.67 &            15.94 \\
5647.01 &            18.79 &            18.67 &            16.39 \\
5486.01 &            18.47 &            18.09 &            13.29 \\
3690.01 &            18.46 &            18.31 &            15.87 \\
1551.01 &            18.16 &            17.91 &            15.09 \\
3754.01 &            18.03 &            17.72 &            13.39 \\
3772.01 &            17.93 &            17.56 &            14.26 \\
3802.01 &            17.74 &            17.55 &            15.15 \\
3679.01 &            17.53 &            17.26 &            13.72 \\
5345.01 &            17.49 &            15.56 &             3.36 \\
5427.01 &            17.11 &            16.83 &            12.44 \\
1596.01 &            16.96 &            16.89 &            15.48 \\
3663.01 &            16.81 &            16.78 &            16.05 \\
5426.01 &            16.78 &            15.83 &             5.68 \\
3899.01 &            16.63 &            16.46 &            14.52 \\
 981.01 &            16.49 &            14.26 &             5.87 \\
3718.01 &            16.40 &            16.05 &            11.30 \\
5646.01 &            15.85 &            14.94 &             5.61 \\
3296.01 &            15.79 &            15.61 &            12.88 \\
3652.01 &            15.50 &            15.43 &            14.22 \\
4074.01 &            15.48 &            15.25 &            12.27 \\
3698.01 &            15.26 &            15.05 &            12.60 \\
5764.01 &            15.05 &            14.93 &            12.74 \\
5468.01 &            14.39 &            14.33 &            12.98 \\
3732.01 &            14.19 &            13.89 &             9.65 \\
5592.01 &            13.72 &            13.52 &            11.03 \\
3688.01 &            13.57 &            13.41 &            11.12 \\
4646.01 &            13.47 &            13.25 &             9.29 \\
5355.01 &            13.17 &            12.94 &             9.12 \\
3720.01 &            13.04 &            12.94 &            11.14 \\
2026.01 &            12.64 &            12.31 &             7.96 \\
5668.01 &            12.44 &            12.23 &             9.57 \\
3877.01 &            11.89 &            11.80 &            10.40 \\
5760.01 &            11.80 &            11.59 &             8.33 \\
5364.01 &            11.38 &            11.29 &             9.77 \\
2791.01 &            11.26 &            11.15 &             9.21 \\
5594.01 &            11.10 &            10.89 &             8.06 \\
5636.01 &            11.02 &            10.04 &             2.83 \\
3694.01 &            10.89 &            10.32 &             6.28 \\
2987.01 &            10.73 &            10.14 &             6.90 \\
5590.01 &            10.56 &             9.38 &             4.91 \\
5649.01 &            10.53 &            10.47 &             9.33 \\
3683.01 &            10.47 &            10.26 &             7.73 \\
5502.01 &            10.34 &             9.92 &             5.29 \\
3761.01 &            10.25 &            10.21 &             9.30 \\
5690.01 &            10.07 &            10.01 &             8.66 \\
5595.01 &            10.00 &             9.47 &             4.33 \\
3696.01 &             9.51 &             9.28 &             6.47 \\
5755.01 &             9.34 &             9.07 &             5.93 \\
3981.01 &             9.25 &             9.14 &             7.22 \\
1560.01 &             9.25 &             9.15 &             7.79 \\
3988.01 &             9.23 &             8.98 &             5.81 \\
1546.01 &             8.58 &             7.25 &             4.46 \\
3668.01 &             8.13 &             8.04 &             6.79 \\
5645.01 &             8.05 &             7.75 &             5.26 \\
5625.01 &             7.84 &             7.04 &             1.84 \\
5113.01 &             7.40 &             7.21 &             5.36 \\
2985.01 &             7.33 &             7.24 &             5.99 \\
3717.01 &             7.33 &             7.28 &             6.66 \\
5580.01 &             7.00 &             6.88 &             5.61 \\
5582.01 &             6.27 &             6.18 &             4.91 \\
5761.01 &             6.10 &             5.99 &             4.48 \\
5776.01 &             5.96 &             5.82 &             4.09 \\
3644.01 &             5.75 &             5.71 &             4.82 \\
1593.01 &             5.27 &             5.22 &             4.33 \\
4001.01 &             5.16 &             5.02 &             3.36 \\
3244.01 &             4.76 &             4.73 &             4.21 \\
5664.01 &             3.41 &             3.35 &             2.61 \\
5599.01 &             3.00 &             2.90 &             1.76 \\
5699.01 &             2.99 &             2.96 &             2.52 \\
5637.01 &             2.83 &             2.80 &             2.17 \\
\bottomrule
\end{tabular}
\end{table}

